COZMIC. I. Cosmological Zoom-in Simulations with Initial Conditions Beyond Cold Dark Matter

We present 72 cosmological dark matter-only $N$-body zoom-in simulations with initial conditions beyond cold, collisionless dark matter (CDM), as the first installment of the COZMIC suite. We simulate Milky Way (MW) analogs with linear matter power spectra $P(k)$ for i) thermal-relic warm dark matter (WDM) with masses $m_{\mathrm{WDM}}\in [3,4,5,6,6.5,10]~\mathrm{keV}$, ii) fuzzy dark matter (FDM) with masses $m_{\mathrm{FDM}}\in [25.9,69.4,113,151,185,490]\times 10^{-22}~\mathrm{eV}$, and iii) interacting dark matter (IDM) with a velocity-dependent elastic proton scattering cross section $\sigma=\sigma_0 v^n$ relative particle velocity scaling $n\in [2,4]$, and dark matter mass $m_{\mathrm{IDM}}\in[10^{-4},~ 10^{-2},~ 1]$ GeV. Subhalo mass function (SHMF) suppression is significantly steeper in FDM versus WDM, while dark acoustic oscillations in $P(k)$ can reduce SHMF suppression for IDM. We fit SHMF models to our simulation results and derive new bounds on WDM and FDM from the MW satellite population, obtaining $m_{\mathrm{WDM}}>5.9~\mathrm{keV}$ and $m_{\mathrm{FDM}}>1.4\times 10^{-20}~\mathrm{eV}$ at $95\%$ confidence; these limits are $\approx 10\%$ weaker and $5\times$ stronger than previous constraints owing to the updated transfer functions and SHMF models, respectively. We estimate IDM bounds for $n=2$ ($n=4$) and obtain $\sigma_0 < 1.0\times 10^{-27}$, $1.3\times 10^{-24}$, and $3.1\times 10^{-23}~\mathrm{cm}^2$ ($\sigma_0 < 9.9\times 10^{-27}$, $9.8\times 10^{-21}$, and $2.1\times 10^{-17}~\mathrm{cm}^2$) for $m_{\mathrm{IDM}}=10^{-4}$, $10^{-2}$, and $1$ GeV, respectively. Thus, future development of IDM SHMF models can improve IDM cross section bounds by up to a factor of $\sim 20$ with current data. COZMIC presents an important step toward accurate small-scale structure modeling in beyond-CDM cosmologies, critical to upcoming observational searches for dark matter physics.

==> hyperlink-year-only-natbib-patch.tex <==
% found on https://tex.stackexchange.com/questions/23227/how-to-hyperlink-only-the-year-part-when-using-natbib-and-hyperref

\RequirePackage{hyperref}
\RequirePackage{natbib}
\RequirePackage{etoolbox}

\makeatletter

% Patch case where name and year are separated by aysep
\patchcmd{\NAT@citex}
  {\@citea\NAT@hyper@{%
     \NAT@nmfmt{\NAT@nm}%
     \hyper@natlinkbreak{\NAT@aysep\NAT@spacechar}{\@citeb\@extra@b@citeb}%
     \NAT@date}}
  {\@citea\NAT@nmfmt{\NAT@nm}%
   \NAT@aysep\NAT@spacechar\NAT@hyper@{\NAT@date}}{}{}

% Patch case where name and year are separated by opening bracket
\patchcmd{\NAT@citex}
  {\@citea\NAT@hyper@{%
     \NAT@nmfmt{\NAT@nm}%
     \hyper@natlinkbreak{\NAT@spacechar\NAT@@open\if*#1*\else#1\NAT@spacechar\fi}%
       {\@citeb\@extra@b@citeb}%
     \NAT@date}}
  {\@citea\NAT@nmfmt{\NAT@nm}%
   \NAT@spacechar\NAT@@open\if*#1*\else#1\NAT@spacechar\fi\NAT@hyper@{\NAT@date}}
  {}{}

\makeatother

